Stable Object Reorientation using Contact Plane Registration

We present a system for accurately predicting stable orientations for diverse rigid objects. We propose to overcome the critical issue of modelling multimodality in the space of rotations by using a conditional generative model to accurately classify contact surfaces. Our system is capable of operating from noisy and partially-observed pointcloud observations captured by real world depth cameras. Our method substantially outperforms the current state-of-the-art systems on a simulated stacking task requiring highly accurate rotations, and demonstrates strong sim2real zero-shot transfer results across a variety of unseen objects on a real world reorientation task. Project website: \url{https://richardrl.github.io/stable-reorientation/}

==> old.tex <==

% We will henceforth refer to the next object to be stacked as the \textbf{source object}. We first generate a set of predicted \textbf{contact points} for the source object by using the $\tt{num\_points} \times 3$ pointcloud and the predicted $\tt{num\_points} \times 1$ contact mask and selecting the pointcloud points with probability $> .5$, according to the contact mask, as the contact points. We fit a plane to this set of contact points using random sampling and consensus (RANSAC) plane segmentation \cite{zhou2018open3d}. RANSAC plane segmentation uniformly samples subsets of inlier points from the full set of contact points, fits planes to each inlier set, then selects the plane with lowest error (e.g. mean squared error, least absolute deviations) to its corresponding inlier set as the optimal plane.

% We frame the problem of aligning two contact planes as applying the relative rotation from the oriented normal of the source object's contact plane to the gravity vector $\begin{bmatrix}0,  0, -1\end{bmatrix}^T$. The sign ambiguity of the contact plane normal vector is addressed by selecting the sign direction that points away from the object center of mass. We assume that the source object will be rotated in the world frame, and that the object is centered at the world frame origin before applying a rotation. Given two contact plane normal vectors, we find the rotation matrix aligning the source vector $\myvec{s}$ to the target vector $\myvec{t}$ using Rodrigues' formula. 

% \pulkit{There is no reconstruction. This needs to come way above in the method}


%In general, the best strategy we converged to during our experiments aligns with recent developments in implicit functions and (Andy Zeng's stuff?), where direct regression or multimodal modelling is less preferred than learning an implicit quantity that can be optimized at test-time. 


% Additionally, we add a KL(p$||$q) regularization term to the KL regularization term, to encourage the prior distribution to more closely match the aggregated posterior \cite{hoffman2016elbo}. \pulkit{This just appears as a side note, cannot do this. Motivate / explain -- refer to proper ML literature}. 



% This capability is essential for determining the affordance of a potential contact region of the object. For example, for determining the optimal contact region, we would like to distinguish between flat regions and curved regions, because placing the object on a flat face is more stable than placing it on a curved region.  \pulkit{No need to explain why DGCNN is better than PointNet, the DGCNN paper did that already -- just state in one line}. 

% The main hyperparameter in DGCNN is $k$, the number of neighboring points considered per input point. We set $k = 20$.

% We briefly discuss the important difference between PointNet and DGCNN. In PointNet, each point in the $\tt{num\_points} \times 3$ input pointcloud is independently projected from $3$ feature dimensions to $1024$ feature dimensions, then max pooled so that points may communicate information to each other in a global manner.  The reason PointNet is not able to compute features describing local geometry effectively is due to a majority of processing in PointNet being done independently for each point. In comparison, DGCNN processes local neighborhoods of points. It accomplishes this by applying an edge convolution operation over fixed-size graphs associated with each point, instead of operating on individual points (like PointNet). The major innovation from DGCNN is the use of k-nearest neighbors to generate fixed-sized local neighborhood graphs per point, instead of generating fully connected graphs like in self-attention. By avoiding the fully connected graph structure, and the resulting quadratic computation in the number of points, DGCNN is able to scale up to much larger point sets than self-attention architectures. Further details may be found in the respective papers \cite{qi2017pointnet} \cite{wang2019dynamic}.


% We make the following contributions:
% \begin{enumerate}
%     \item We show that a learning based approach is able to overcome noise and occlusions where previous approaches based on mesh reconstruction fail, while also having the capability to generalize to new objects.
%     % \item We show that, in order to obtain good accuracy while matching the modes, utilizing a higher $\beta$ constant is necessary, and the multimodal prior is required for simultaneously low reconstruction and KL regularization error
%     % \item We show that crippling the decoder is necessary to avoid posterior collapse, and introduce a simple encoder/decoder parameterization of PointNet to enable this crippling. 
%     % \pulkit{Dont say crippling, but reducing the capacity.}
%     % \item We show that modelling relative rotations instead of predicting the object pose leads to better object generalization 
%     % \pulkit{There is no such thing as an absolute pose anyways}
%     \item We show that a classification-based registration method outperforms direct rotation representation regression and an oriented bounding box baseline.
%     \item We propose several specific techniques to improve the accuracy of the classification-based method, such that we can stack towers of 4+ blocks with high accuracy.
% \end{enumerate}



%\begin{enumerate}
    %\item It is difficult to accurately regress rotation representations, especially when rotation magnitudes are large. We reframe the orientation prediction problem as a classification and registration problem, and show that our approach vastly outperforms direct rotation regression, which is often unable to converge during training.

    % By performing this procedure, we avoid the difficult problem of directly regressing 3D rotations. 
    
    % \item By utilizing pointcloud processing architectures and a registration method based on plane fitting and alignment, we are able to be more robust to noise and occlusion. \pulkit{Are there specific architecture that work better? The alignment part belongs to the first part.}
%\end{enumerate}
% assume object categories and category-level poses (thereby hindering inter-category generalization) \cite{kulkarni2019unsupervised, manuelli2019kpam, nagabandi2020deep, liu2020keypose, }, 


% Regression is hard. We can classify rotations into buckets. But there is a problem. No notion of distance between the classes. Lucas Manuelli average over buckets. Pixels. Tune the averaging neighborhood. Keypoint regression. If buckets are too coarse, averaging is not precise. 

% Too many buckets, cannot share data between buckets.

% If you classify points, you can get highly accurate continuous rotations. Binary classifcation vs multiclass classification (discrete rotations). Less knowledge sharing.  

% We motivate this method with the intuition that classifying the segmentation mask may be easier than regressing a rotation, since successful binary classification only requires the relative value of each logit to be appropriately thresholded into the right class \pulkit{unclear what is relative value of logit, appropriately thresholded means or what is the right class}, whereas successful rotation regression requires predicting each rotation representation parameter to a high degree of accuracy \pulkit{Why is that not the case with predicting the segmentation mask?}.

% This motivates the need for a generative model for producing the contact masks.

% However, an approach based on classifying contact regions is affected by multimodality due to reflectional symmetry, whereas explicit rotation regression is not. 


% \subsection{Learning a Contact Mask with Conditional VAE}
% How much to describe here? Reproducing CVAE seems a bit wasteful. Put in appendix?
% \pulkit{Are there any particular insights you have about the conditional VAE or innovations that work better?. At the bare minimum it is necessary to formalize the inputs / outputs. Probably formalize the previous paragraph with symbols, write down the loss function etc.} 


% We additionally make several modifications to our CVAE to improve performance. We use the standard technique of annealing the $\beta$-parameter, which trades off the reconstruction and Kullback Leibler (KL) regularization error KL(q$||$p), from $0$ to $.02$ according to the following sigmoidal annealing schedule: . We use a Mixture of Gaussians (MoG) prior to improve the evidence lower bound (ELBO) optimization, and found empirically that adding more components to the MoG prior lead to lower convergent KL regularization error. Our final model uses five MoG components. We also fix the variance of the prior. 
% \pulkit{This belongs to the CVAE section of the paper; does MoG actually help?}.


% How can we reframe rotation prediction as a classification problem? 
%Given the challenges of directly predicting rotation matrices as described above, we propose  to estimate stacking rotations through the intermediate step of contact plane registration. Imagine we have an object lying in an arbitrary orientation on the table that we want to stack. We denote this object as the source object. First, we must identify a subset of points on the source object that we believe should be in contact with either the top of the table or the top of an existing tower of objects (some top surface). We fit a plane to these contact points, then align that plane with the aforementioned top surface. 

% \subsection{Results Outline (To be removed)}
% \begin{enumerate}
%     \item Shape generalization
%     \begin{enumerate}
%         \item Good augmentation
%         \item Good architecture (Make comparison between DGCNN + PointNet)
%     \end{enumerate}
%     \item Noise
%     \begin{enumerate}
%         \item RANSAC plane seg (Make comparison between RANSAC plane seg and ICP)
%     \end{enumerate}
%     \item Occlusion
%     \begin{enumerate}
%         \item Linear search for the best set of contact points (Make comparison between linear search with a .02 / .04 threshold frac contact region and a .04 threshold frac starting from the minimum object height)
%     \end{enumerate}
%     \item Accuracy / unimodality of predicted contact masks
%     \begin{enumerate}
%         \item All of the above
%         \item Better masks
%         \begin{enumerate}
%             \item Precision-recall trade-off parameter $r$ (Make comparison with r = 2 vs r =4 for the best model)
%             \item KLD term (Make comparison with .02 term and without) 
%             \item Mixture of Gaussians (Make comparison with 1 component vs 5 component [low priority])
%         \end{enumerate}
%     \end{enumerate}
% \end{enumerate}

% Remaining experiments (low priority)
% \begin{enumerate}
%     \item No CVAE + plane segmentation (might work pretty well... uh oh...)
% \end{enumerate}

%\subsection{Face segmentation + scoring faces} We could also segment the faces with repeated RANSAC plane segmentation, then learn a set predictor that predicts which of the faces is the best one, then apply our procedure in \ref{Contact plane registration} to acquire a relative rotation. Compared to this approach, we predict a subset of the points with a neural network before fitting the RANSAC plane segmentation. Our approach should be able to find better results (Should we even include this section? Full experiments will be a hassle/no time. But we could show individual examples of why plane segmentation on the full pointcloud often leads to bad results.). 


% \subsection{Stacking policy} In order to stack an object on top of the existing tower or table, the following procedure is applied. First, we decide which object to stack next. Then, we take the pointcloud of the currently-stacking object in the world frame, and subtract its center of mass, such that the object is now centered at the world frame origin. Next, we apply the relative rotation found according to \ref{Contact plane registration} to get the object in the right orientation. Next, we translate the object downwards until it comes in contact with an object, before stopping and placing the object. Out of all these steps, only the relative rotation is predicted and learned. The remaining parts come from a scripted policy that assumes access to ground truth center of mass (but not orientation). Existing works may be applied to predict the object center of mass from pointcloud observation \cite{qi2019deep}. 




% The reason being, in order for an object which is being stacked to remain stable after being stacked, its center of mass must lie within the support polygon between it and the object we are stacking upon. The support polygon is the ``footprint" between two stacked objects.
% It is worth noting that in the scenario where one object is stacked on top of other, only aligning surface normals of the contact and placement surface may not result in the maximally stable configuration. This is because, depending on the shape of two blocks  depending on the shape of the different stable rotations about the $Z$ axis

% To maximize stability, we would like to pick the planar orientation that maximizes the area of the support polygon. The support polygon is the convex hull of the contact points of the object projected onto the top of the tower or table.



%\subsection{Learning the Distribution of Contact Masks}
%\label{sec:contact-plane-prediction}


% Given the multimodality in the label space of contact masks, as discussed in Sec. \ref{sec:object_datasets_and_shape_generalization}, we first used conditional VAE (CVAE) to learn a distribution of contact masks. We performed extensive hyperparameter tuning over the prior and the $\beta$-weighting parameter \cite{higgins2016beta}. The problem was there was no value of the $\beta$-parameter we could find that could optimize both the reconstruction loss and KL regularization loss to an acceptable level such that the contact masks predicted at test-time were accurate enough for consistent success at the stacking. Additionally, we observed a phenomenon where object types that should have only one contact mask, were instead associated with multiple contact masks as new latents were sampled from the prior at test-time. This phenomenon likely occurs due to the distribution mismatch between the aggregate posterior seen by the decoder during training \cite{hoffman2016elbo} and the prior distribution seen by the decoder during testing, as well as the presence of both multimodal and unimodal objects in the training dataset. We report the performance of the best performing CVAE model in Sec. \ref{sec:results}. 

% We eventually found a solution that was much easier to train and that required significantly less hyperparameter tuning. Instead of learning a generative model, we simply learn a classifier which predicts contact masks given pointcloud input. A classifier will naturally handle multimodality by averaging the logits. The resulting contact mask logits will be proportional to the union of contact masks seen in the training set labels. 

% Given this union of contact masks, where each mask is associated with a plane, how do we retrieve a single plane? We found that the RANSAC plane segmentation is able to perform this retrieval correctly and with a high degree of accuracy. 


% We first take the pointcloud of the object in the starting orientation $R_s$, and apply the inverse of the relative orientation from start to target: $R_r^{-1} = (R_t R_s)^{-1}$. This rotation rotates our noisy, occluded pointcloud into the stacked orientation, at which point we can easily segment the contact points according to a simple rule: take the bottom $\tt{threshold\_frac} \in (0, 1)$ points, according to the points' z-axis values, as contact points. The contact points are thus all points on the observed pointcloud that fall within two planes that are orthogonal to the gravity vector and whose distance between them is $\tt{threshold\_frac} \cdot \tt{object\_height}$. 

% When an object is in the stacked orientation, the object ``bottom" is consistently defined across object types relative to the world-frame z-axis. 

% \pulkit{How do we know what is the bottom}.

% \pulkit{How exactly do you do the scoring? This seems like a voting scheme -- cite the appropriate ML literature}.
% While simple, this procedure has an issue. It is often the case that the bottom $\tt{threshold\_frac}$ points may not correctly fit a plane. The bottom $\tt{threshold\_frac}$ corresponds to a threshold interval of $[0, \tt{threshold\_frac}]$. Instead of using a threshold interval starting at $0$ and ending at $\tt{threshold\_frac}$, we perform a line search over other threshold intervals up to some maximal upper bound (we set this to $10\%$). At each threshold interval, we fit a plane to the contact points falling within the threshold interval. We then calculate the rotation angle between the oriented plane normal and the gravity vector, and select the plane and corresponding threshold interval that minimizes this rotation angle. In the ideal case, we should be able to find a slice of contact points such that a plane fit over these contact points is perfectly orthogonal with the gravity vector. We select points contained within the optimal threshold interval as the contact points for each sample.


% While simple, this procedure has an issue. It is often the case that the bottom $\tt{threshold\_frac}$ points may not correctly fit a plane. The bottom $\tt{threshold\_frac}$ corresponds to a threshold interval of $[0, \tt{threshold\_frac}]$. Instead of using a threshold interval starting at $0$ and ending at $\tt{threshold\_frac}$, we perform a line search over other threshold intervals up to some maximal upper bound (we set this to $10\%$). At each threshold interval, we fit a plane to the contact points falling within the threshold interval. We then calculate the rotation angle between the oriented plane normal and the gravity vector, and select the plane and corresponding threshold interval that minimizes this rotation angle. In the ideal case, we should be able to find a slice of contact points such that a plane fit over these contact points is perfectly orthogonal with the gravity vector. We select points contained within the optimal threshold interval as the contact points for each sample.


==> results_backup.tex <==

\section{Results}
\label{results_section}
\subsection{Results Outline (To be removed)}
\begin{enumerate}
    \item Shape generalization
    \begin{enumerate}
        \item Good augmentation
        \item Good architecture (Make comparison between DGCNN + PointNet)
    \end{enumerate}
    \item Noise
    \begin{enumerate}
        \item RANSAC plane seg (Make comparison between RANSAC plane seg and ICP)
    \end{enumerate}
    \item Occlusion
    \begin{enumerate}
        \item Linear search for the best set of contact points (Make comparison between linear search with a .02 / .04 threshold frac contact region and a .04 threshold frac starting from the minimum object height)
    \end{enumerate}
    \item Accuracy / unimodality of predicted contact masks
    \begin{enumerate}
        \item All of the above
        \item Better masks
        \begin{enumerate}
            \item Precision-recall trade-off parameter $r$ (Make comparison with r = 2 vs r =4 for the best model)
            \item KLD term (Make comparison with .02 term and without) 
            \item Mixture of Gaussians (Make comparison with 1 component vs 5 component [low priority])
        \end{enumerate}
    \end{enumerate}
\end{enumerate}

Remaining experiments (low priority)
\begin{enumerate}
    \item No CVAE + plane segmentation (might work pretty well... uh oh...)
\end{enumerate}

% \begin{table*}[t]
% \caption{Stacking Success Rates for Two Object Towers over 100 Trials Each}
% \label{table_example}
% \begin{center}
% \begin{tabular}{|c||c|c|c|c|}
% \hline
% Second Object Name & Ours & OBB & Plane Seg & CVAE + Quat \\
% \hline
% Barrell & \textbf{0.85} & 0.82\\
% \hline
% Bridge & 0.91 & \textbf{0.93}\\
% \hline
% Egg & \textbf{0.37} & 0.29\\
% \hline
% J Block & \textbf{0.43} & 0.19\\
% \hline
% L Chamfered & \textbf{0.79} & 0.56\\
% \hline
% Nut & \textbf{0.72} & 0.36\\
% \hline
% Pyramid w/ Eye & \textbf{0.97} & 0.47\\
% \hline
% Vase w/ Hole & \textbf{0.84} & 0.34\\
% \hline
% Block & 0.99 & \textbf{1.0}\\
% \hline
% Cone & \textbf{0.98} & 0.22\\
% \hline
% Cone + Ball & \textbf{0.77} & 0.58\\
% \hline
% Cross & \textbf{0.89} & 0.58\\
% \hline
% Cross Round Top & \textbf{0.77} & 0.45\\
% \hline
% Cylinder Long & 0.38 & \textbf{0.97}\\
% \hline
% Cylinder Parallelogram & \textbf{0.98} & 0.02\\
% \hline
% Foundation & 0.88 & \textbf{0.99}\\
% \hline
% Pentagram Stout & \textbf{0.94} & 0.13\\
% \hline
% Rectangular Solid & 0.7 & \textbf{0.99}\\
% \hline
% Rounded Bobble & 0.05 & \textbf{0.32}\\
% \hline
% Wedge Long & \textbf{0.7} & 0.19\\
% \hline
% Wedge Short Stout & \textbf{0.86} & 0.2\\
% \hline
% \end{tabular}
% \end{center}
% \end{table*}

\begin{table*}[t]
\centering
\label{stacking_succ_rate_table}
\caption{Stacking Success Rates and Angular Errors for Two Object Towers (NOTE: REMOVE THIS MESSAGE UPON THE FINAL VERSION, AND MAKE SURE THE OBJECT NAMES ARE SPELLED NICELY)}
% \begin{tabular}{llll}
% \toprule
% {} &              Oriented Bounding Box &     Plane Segmentation &                               Contact Mask Union + Plane Seg \\
% \midrule
% Barrell              &              0.72 (0.18$\pm$0.21)  &    0.0 (1.4$\pm$0.29)  &   $\mathbf{0.99}$ (0.053$\pm$0.03) \\
% Block                &   $\mathbf{1.0}$ (0.051$\pm$0.029) &  0.14 (0.42$\pm$0.64)  &            0.99 (0.038$\pm$0.022)  \\
% Bridge               &             0.92 (0.054$\pm$0.03)  &   0.03 (1.4$\pm$0.42)  &  $\mathbf{0.97}$ (0.034$\pm$0.021) \\
% Cone                 &                0.29 (1.9$\pm$1.3)  &  0.11 (0.41$\pm$0.71)  &   $\mathbf{1.0}$ (0.032$\pm$0.019) \\
% Cone+ball            &                0.46 (1.8$\pm$1.5)  &    0.0 (1.6$\pm$0.35)  &  $\mathbf{0.97}$ (0.046$\pm$0.027) \\
% Cross                &              0.59 (0.65$\pm$0.61)  &   0.1 (1.5$\pm$0.085)  &    $\mathbf{0.94}$ (0.17$\pm$0.42) \\
% Cross round top      &               0.4 (0.77$\pm$0.53)  &  0.07 (0.85$\pm$0.69)  &    $\mathbf{0.92}$ (0.14$\pm$0.36) \\
% Cylinder long        &  $\mathbf{0.97}$ (0.022$\pm$0.012) &   0.0 (1.5$\pm$0.031)  &              0.38 (0.12$\pm$0.19)  \\
% Cylinder parallogram &             0.02 (0.48$\pm$0.051)  &   0.03 (1.1$\pm$0.48)  &   $\mathbf{1.0}$ (0.048$\pm$0.028) \\
% Egg                  &                0.35 (1.5$\pm$1.4)  &    0.03 (1.6$\pm$0.2)  &    $\mathbf{0.69}$ (0.45$\pm$0.71) \\
% Foundation           &  $\mathbf{0.99}$ (0.048$\pm$0.029) &   0.03 (1.3$\pm$0.55)  &            0.93 (0.052$\pm$0.032)  \\
% J block              &                0.23 (1.5$\pm$1.1)  &    0.0 (1.5$\pm$0.28)  &    $\mathbf{0.85}$ (0.21$\pm$0.48) \\
% L chamfered          &                0.48 (1.7$\pm$1.4)  &  0.09 (0.73$\pm$0.76)  &    $\mathbf{1.0}$ (0.084$\pm$0.26) \\
% Nut                  &              0.26 (0.36$\pm$0.11)  &    0.0 (1.3$\pm$0.17)  &     $\mathbf{0.81}$ (0.3$\pm$0.56) \\
% Pentagram stout      &               0.19 (0.4$\pm$0.15)  &   0.14 (1.4$\pm$0.14)  &     $\mathbf{0.96}$ (0.3$\pm$0.54) \\
% Pyramid w eye        &               0.37 (0.78$\pm$0.2)  &  0.13 (0.13$\pm$0.18)  &   $\mathbf{1.0}$ (0.051$\pm$0.033) \\
% Rectangular solid    &  $\mathbf{0.64}$ (0.027$\pm$0.013) &    0.0 (1.5$\pm$0.23)  &            0.34 (0.078$\pm$0.041)  \\
% Rounded bobble       &      $\mathbf{0.33}$ (1.9$\pm$1.3) &    0.0 (1.5$\pm$0.32)  &                0.32 (1.0$\pm$1.0)  \\
% Vase w hole          &               0.26 (0.8$\pm$0.55)  &  0.08 (0.84$\pm$0.57)  &   $\mathbf{0.94}$ (0.087$\pm$0.17) \\
% Wedge long           &                0.15 (1.7$\pm$1.3)  &  0.05 (0.98$\pm$0.78)  &   $\mathbf{0.93}$ (0.065$\pm$0.16) \\
% Wedge short stout    &               0.24 (1.1$\pm$0.63)  &  0.01 (0.29$\pm$0.52)  &    $\mathbf{0.92}$ (0.75$\pm$0.75) \\
% \bottomrule
% \end{tabular}
% \begin{tabular}{lllll}
% \toprule
% {} &              Oriented BB &     Multi-plane Seg & CVAE+CM+MoG5 &                               Union of CM+Plane Seg \\
% \midrule
% Barrell              &              0.72 (0.18$\pm$0.21)  &    0.0 (1.4$\pm$0.29)  &                  0.75 (0.28$\pm$0.46)  &   $\mathbf{0.99}$ (0.053$\pm$0.03) \\
% Block                &   $\mathbf{1.0}$ (0.051$\pm$0.029) &  0.14 (0.42$\pm$0.64)  &                0.93 (0.046$\pm$0.029)  &            0.99 (0.038$\pm$0.022)  \\
% Bridge               &             0.92 (0.054$\pm$0.03)  &   0.03 (1.4$\pm$0.42)  &                0.83 (0.046$\pm$0.025)  &  $\mathbf{0.97}$ (0.034$\pm$0.021) \\
% Cone                 &                0.29 (1.9$\pm$1.3)  &  0.11 (0.41$\pm$0.71)  &                  0.95 (0.06$\pm$0.18)  &   $\mathbf{1.0}$ (0.032$\pm$0.019) \\
% Cone+ball            &                0.46 (1.8$\pm$1.5)  &    0.0 (1.6$\pm$0.35)  &                  0.75 (0.39$\pm$0.89)  &  $\mathbf{0.97}$ (0.046$\pm$0.027) \\
% Cross                &              0.59 (0.65$\pm$0.61)  &   0.1 (1.5$\pm$0.085)  &                  0.87 (0.26$\pm$0.53)  &    $\mathbf{0.94}$ (0.17$\pm$0.42) \\
% Cross round top      &               0.4 (0.77$\pm$0.53)  &  0.07 (0.85$\pm$0.69)  &                  0.71 (0.45$\pm$0.67)  &    $\mathbf{0.92}$ (0.14$\pm$0.36) \\
% Cylinder long        &  $\mathbf{0.97}$ (0.022$\pm$0.012) &   0.0 (1.5$\pm$0.031)  &                  0.24 (0.31$\pm$0.45)  &              0.38 (0.12$\pm$0.19)  \\
% Cylinder parallogram &             0.02 (0.48$\pm$0.051)  &   0.03 (1.1$\pm$0.48)  &                0.96 (0.048$\pm$0.099)  &   $\mathbf{1.0}$ (0.048$\pm$0.028) \\
% Egg                  &                0.35 (1.5$\pm$1.4)  &    0.03 (1.6$\pm$0.2)  &                   0.33 (1.0$\pm$0.89)  &    $\mathbf{0.69}$ (0.45$\pm$0.71) \\
% Foundation           &  $\mathbf{0.99}$ (0.048$\pm$0.029) &   0.03 (1.3$\pm$0.55)  &                 0.81 (0.097$\pm$0.22)  &            0.93 (0.052$\pm$0.032)  \\
% J block              &                0.23 (1.5$\pm$1.1)  &    0.0 (1.5$\pm$0.28)  &                    0.41 (1.0$\pm$1.0)  &    $\mathbf{0.85}$ (0.21$\pm$0.48) \\
% L chamfered          &                0.48 (1.7$\pm$1.4)  &  0.09 (0.73$\pm$0.76)  &                   0.75 (0.99$\pm$1.4)  &    $\mathbf{1.0}$ (0.084$\pm$0.26) \\
% Nut                  &              0.26 (0.36$\pm$0.11)  &    0.0 (1.3$\pm$0.17)  &                  0.68 (0.38$\pm$0.61)  &     $\mathbf{0.81}$ (0.3$\pm$0.56) \\
% Pentagram stout      &               0.19 (0.4$\pm$0.15)  &   0.14 (1.4$\pm$0.14)  &                  0.84 (0.14$\pm$0.35)  &     $\mathbf{0.96}$ (0.3$\pm$0.54) \\
% Pyramid w eye        &               0.37 (0.78$\pm$0.2)  &  0.13 (0.13$\pm$0.18)  &                0.97 (0.059$\pm$0.088)  &   $\mathbf{1.0}$ (0.051$\pm$0.033) \\
% Rectangular solid    &  $\mathbf{0.64}$ (0.027$\pm$0.013) &    0.0 (1.5$\pm$0.23)  &                  0.39 (0.16$\pm$0.35)  &            0.34 (0.078$\pm$0.041)  \\
% Rounded bobble       &      $\mathbf{0.33}$ (1.9$\pm$1.3) &    0.0 (1.5$\pm$0.32)  &                    0.18 (1.3$\pm$0.9)  &                0.32 (1.0$\pm$1.0)  \\
% Vase w hole          &               0.26 (0.8$\pm$0.55)  &  0.08 (0.84$\pm$0.57)  &                   0.8 (0.24$\pm$0.34)  &   $\mathbf{0.94}$ (0.087$\pm$0.17) \\
% Wedge long           &                0.15 (1.7$\pm$1.3)  &  0.05 (0.98$\pm$0.78)  &                  0.65 (0.54$\pm$0.73)  &   $\mathbf{0.93}$ (0.065$\pm$0.16) \\
% Wedge short stout    &               0.24 (1.1$\pm$0.63)  &  0.01 (0.29$\pm$0.52)  &                  0.85 (0.78$\pm$0.76)  &    $\mathbf{0.92}$ (0.75$\pm$0.75) \\
% \bottomrule
% \end{tabular}
% \begin{tabular}{llllll}
% \toprule
% {} &                        Oriented BB &        Multi-plane Seg &               CVAE+Quat &             CVAE+CM+MoG5 &              Union of CM+Plane Seg \\
% \midrule
% Barrell              &              0.72 (0.18$\pm$0.21)  &    0.0 (1.4$\pm$0.29)  &   0.03 (0.68$\pm$0.41)  &    0.75 (0.28$\pm$0.46)  &   $\mathbf{0.99}$ (0.053$\pm$0.03) \\
% Block                &   $\mathbf{1.0}$ (0.051$\pm$0.029) &  0.14 (0.42$\pm$0.64)  &   0.03 (0.67$\pm$0.38)  &  0.93 (0.046$\pm$0.029)  &            0.99 (0.038$\pm$0.022)  \\
% Bridge               &             0.92 (0.054$\pm$0.03)  &   0.03 (1.4$\pm$0.42)  &    0.0 (0.94$\pm$0.32)  &  0.83 (0.046$\pm$0.025)  &  $\mathbf{0.97}$ (0.034$\pm$0.021) \\
% Cone                 &                0.29 (1.9$\pm$1.3)  &  0.11 (0.41$\pm$0.71)  &  0.03 (0.24$\pm$0.073)  &    0.95 (0.06$\pm$0.18)  &   $\mathbf{1.0}$ (0.032$\pm$0.019) \\
% Cone+ball            &                0.46 (1.8$\pm$1.5)  &    0.0 (1.6$\pm$0.35)  &      0.0 (1.3$\pm$1.0)  &    0.75 (0.39$\pm$0.89)  &  $\mathbf{0.97}$ (0.046$\pm$0.027) \\
% Cross                &              0.59 (0.65$\pm$0.61)  &   0.1 (1.5$\pm$0.085)  &    0.0 (0.98$\pm$0.35)  &    0.87 (0.26$\pm$0.53)  &    $\mathbf{0.94}$ (0.17$\pm$0.42) \\
% Cross round top      &               0.4 (0.77$\pm$0.53)  &  0.07 (0.85$\pm$0.69)  &    0.01 (0.88$\pm$0.3)  &    0.71 (0.45$\pm$0.67)  &    $\mathbf{0.92}$ (0.14$\pm$0.36) \\
% Cylinder long        &  $\mathbf{0.97}$ (0.022$\pm$0.012) &   0.0 (1.5$\pm$0.031)  &    0.01 (0.61$\pm$0.4)  &    0.24 (0.31$\pm$0.45)  &              0.38 (0.12$\pm$0.19)  \\
% Cylinder parallogram &             0.02 (0.48$\pm$0.051)  &   0.03 (1.1$\pm$0.48)  &     0.0 (0.9$\pm$0.35)  &  0.96 (0.048$\pm$0.099)  &   $\mathbf{1.0}$ (0.048$\pm$0.028) \\
% Egg                  &                0.35 (1.5$\pm$1.4)  &    0.03 (1.6$\pm$0.2)  &     0.0 (1.4$\pm$0.73)  &     0.33 (1.0$\pm$0.89)  &    $\mathbf{0.69}$ (0.45$\pm$0.71) \\
% Foundation           &  $\mathbf{0.99}$ (0.048$\pm$0.029) &   0.03 (1.3$\pm$0.55)  &     0.0 (1.1$\pm$0.33)  &   0.81 (0.097$\pm$0.22)  &            0.93 (0.052$\pm$0.032)  \\
% J block              &                0.23 (1.5$\pm$1.1)  &    0.0 (1.5$\pm$0.28)  &   0.08 (0.43$\pm$0.31)  &      0.41 (1.0$\pm$1.0)  &    $\mathbf{0.85}$ (0.21$\pm$0.48) \\
% L chamfered          &                0.48 (1.7$\pm$1.4)  &  0.09 (0.73$\pm$0.76)  &    0.05 (0.5$\pm$0.35)  &     0.75 (0.99$\pm$1.4)  &    $\mathbf{1.0}$ (0.084$\pm$0.26) \\
% Nut                  &              0.26 (0.36$\pm$0.11)  &    0.0 (1.3$\pm$0.17)  &   0.01 (0.51$\pm$0.21)  &    0.68 (0.38$\pm$0.61)  &     $\mathbf{0.81}$ (0.3$\pm$0.56) \\
% Pentagram stout      &               0.19 (0.4$\pm$0.15)  &   0.14 (1.4$\pm$0.14)  &     0.0 (0.51$\pm$0.2)  &    0.84 (0.14$\pm$0.35)  &     $\mathbf{0.96}$ (0.3$\pm$0.54) \\
% Pyramid w eye        &               0.37 (0.78$\pm$0.2)  &  0.13 (0.13$\pm$0.18)  &   0.01 (0.69$\pm$0.24)  &  0.97 (0.059$\pm$0.088)  &   $\mathbf{1.0}$ (0.051$\pm$0.033) \\
% Rectangular solid    &  $\mathbf{0.64}$ (0.027$\pm$0.013) &    0.0 (1.5$\pm$0.23)  &    0.0 (0.59$\pm$0.35)  &    0.39 (0.16$\pm$0.35)  &            0.34 (0.078$\pm$0.041)  \\
% Rounded bobble       &      $\mathbf{0.33}$ (1.9$\pm$1.3) &    0.0 (1.5$\pm$0.32)  &     0.0 (1.4$\pm$0.74)  &      0.18 (1.3$\pm$0.9)  &                0.32 (1.0$\pm$1.0)  \\
% Vase w hole          &               0.26 (0.8$\pm$0.55)  &  0.08 (0.84$\pm$0.57)  &    0.0 (0.94$\pm$0.42)  &     0.8 (0.24$\pm$0.34)  &   $\mathbf{0.94}$ (0.087$\pm$0.17) \\
% Wedge long           &                0.15 (1.7$\pm$1.3)  &  0.05 (0.98$\pm$0.78)  &   0.07 (0.27$\pm$0.18)  &    0.65 (0.54$\pm$0.73)  &   $\mathbf{0.93}$ (0.065$\pm$0.16) \\
% Wedge short stout    &               0.24 (1.1$\pm$0.63)  &  0.01 (0.29$\pm$0.52)  &    0.0 (0.58$\pm$0.32)  &    0.85 (0.78$\pm$0.76)  &    $\mathbf{0.92}$ (0.75$\pm$0.75) \\
% \bottomrule
% \end{tabular}
\end{table*}


% Ours (r=2, linear search, threshold_frac=.02): royalbrook1975_checkpt50
% Ours (r=4, linear search, threshold_frac=.04): 

% \pulkit{Baselines / Evaluation should be moved to the Experimental Setup.}


% Following prior work \cite{mousavian20196}, we set the latent dimension to a small value of $k = 2$ to prevent overfitting to the training set. 

% To find the contact face from the PCA OBB, we select the contact face by inverting the oriented bounding box rotation and choosing the contact face which is orthogonal to the principal axis and whose centroid is positive (thereby choosing one out of the two antiparallel faces). 

% \subsection{Face segmentation + scoring faces} We could also segment the faces with repeated RANSAC plane segmentation, then learn a set predictor that predicts which of the faces is the best one, then apply our procedure in \ref{Contact plane registration} to acquire a relative rotation. Compared to this approach, we predict a subset of the points with a neural network before fitting the RANSAC plane segmentation. Our approach should be able to find better results (Should we even include this section? Full experiments will be a hassle/no time. But we could show individual examples of why plane segmentation on the full pointcloud often leads to bad results.). 


% \subsection{Stacking policy} In order to stack an object on top of the existing tower or table, the following procedure is applied. First, we decide which object to stack next. Then, we take the pointcloud of the currently-stacking object in the world frame, and subtract its center of mass, such that the object is now centered at the world frame origin. Next, we apply the relative rotation found according to \ref{Contact plane registration} to get the object in the right orientation. Next, we translate the object downwards until it comes in contact with an object, before stopping and placing the object. Out of all these steps, only the relative rotation is predicted and learned. The remaining parts come from a scripted policy that assumes access to ground truth center of mass (but not orientation). Existing works may be applied to predict the object center of mass from pointcloud observation \cite{qi2019deep}. 
  
 \subsection{Stacking Evaluation} To evaluate the accuracy of our relative rotation predictions, we use our learned rotation predictor, as well as various baselines, within a hand-scripted stacking policy to build towers from multiple objects on a table. The policy is described in Appendix \ref{stacking_policy}. Our method, as well as the baselines, all operate from noisy, occluded pointclouds of the objects, which have been rendered by the PyBullet depth cameras. We drop the objects randomly on the table, so the rotation function is forced to generalize over unseen starting orientations compared to the training set. All results in this section are evaluated over the set of Bausack test objects, despite the training data coming entirely from the Bandu game objects. We seek to answer the following questions:
\begin{enumerate}
    \item How does the performance of our classification-based registration method compare with direct rotation regression and geometric baselines?
    \item How do various architectural choices affect the performance of our classification-based method?
    \item How successfully can our system generalize over realistic noise, occlusion, and new object geometries?
\end{enumerate}

The policy rollouts are scored according to a step-wise reward function that rewards $+1$ for every stacked object that achieves equal or higher change-in-height (after running forward simulation for 500 timesteps) of the tower compared to the ground truth labelled orientation. If the total reward is equal to the number of objects in the scene, the episode is deemed a success.

We additionally report a more granular quantitative metric - the minimum angular error between normals (\textbf{MAEN}). The purpose of this metric is to quantify the orientation of the contact plane normal of the top object. We label all the ground truth contact planes by specifying a list of oriented contact plane normals for each symmetric object. For each policy rollout, we take the argmin normal out of this list that has the closest rotation angle to the gravity vector, and then report that rotation angle $\theta$. The mean and standard deviation of the MAEN are included in the parentheses in Table \ref{stacking_succ_rate_table}.

% We also show results where both faces are selected.

\subsection{PCA Oriented Bounding Box Baseline} PCA is commonly used to compute bounding boxes for point sets in $\mathbb{R}^n$ \cite{dimitrov2006bounding}. Given an oriented bounding box (OBB), we choose one of the antipodal faces along the longest axis as the ``contact face" and align this contact face with the top of the existing tower or the table, using the same method of aligning contact normals found in Appendix $\ref{Rodrigues'_rot_2_vecs}$.\footnote{The face is chosen via change of basis and selecting the face whose normal point along the positive axis.} While simple, this approach is unable to correctly find the contact face for many object geometries. One reason why the PCA approach fails is because the maximal eigenvector found in PCA is often not orthogonal to a stable contact face. Additionally, PCA may fail when the points are not uniformly sampled from the object surface \cite{dimitrov2006bounding}. (Show image of 3D rhombus? Point density effect on PCA?). 

\subsection{Multi-plane Segmentation \& Height Maximization Baseline} Another baseline we may try is performing multi-plane segmentation by repeatedly applying RANSAC plane segmentation and removing the inlier set from the pointcloud after each segmentation. Once we get a set of potential contact planes, we reorient each plane such that the plane's oriented normal is aligned with the gravity vector, and pick the orientation that maximizes the height of the observed pointcloud. We find that this method fails because running RANSAC plane segmentation on the entire pointcloud usually does not find the true planes of the underlying mesh, and instead finds planes that cut through the interior of the mesh. This motivates our method, which uses learning to fit RANSAC plane segmentation to a subset of points.

\subsection{CVAE with Quaternions Baseline}
\label{cvae_quat_baseline}
We would like to understand how our classification-based approach compares with an approach that directly regresses a rotation representation, i.e. quaternions. Instead of attempting to reconstruct contact masks in the decoder of our CVAE, we reconstruct quaternions. To predict quaternions, our decoder predicts a 4D unit-norm vector. This unit quaternion is analytically converted to a rotation matrix, which can then be regressed against the ground truth rotation matrix via the ``chordal" loss \cite{peretroukhin2020smooth}:
% $$d_{\text{chord}} (R_{\text{pred}}, R_{\text{gt}}) = || R_{\text{pred}} - R_{\text{gt}}||_F$$
$\mathcal{L_{\text{recon}}} (R_{\text{pred}}, R_{\text{gt}}) = || R_{\text{pred}} - R_{\text{gt}}||_F$ 

This baseline produces poor results because we are unable to find a good value for $\beta$ that simultaneously minimizes the reconstruction and KL divergence loss. We hypothesize one reason for the optimization difficulty is due to the independent latent variables having a difficult time modelling the highly dependent orientation information. Improving the posterior or prior with normalizing flows, which are architecturally better suited for producing dependent latent variables, may be one promising way to improve explicit rotation prediction with conditional generative models \cite{rezende2015variational}. 

\subsection{Direct Quaternion Prediction Baseline}
We consider two baselines. The first, we directly predict the quaternion given pointcloud input, using the quaternion representation from \cite{peretroukhin2020smooth}, analytically converting the quaternion to a rotation matrix, and applying the chordal loss mentioned in Sec. \ref{cvae_quat_baseline}. The model was unable to make significant learning progress after 15 hours of training on the full of Bandu objects. To sanity check our architecture and loss, we pull out the five objects from the Bandu training set without rotational symmetry and train our model only on this subset. The model is again unable to train when applying full XYZ rotation augmentation. We also try the ShapeMatchLoss \cite{xiang2017posecnn}, which regresses distances between closest points instead of directly regressing rotation representations. However, as in prior work \cite{devgon2020orienting}, we observe difficulties in optimizing the ShapeMatchLoss, and are unable to make significant learning progress.

\subsection{Quantitative and Qualitative Analysis} 
Our first experiment compares the performance of various methods for generating the relative rotation. We evaluate across 100 trials, for each object type, the task of building two-object towers. The first object to be stacked in this experiment is always the ``Foundation" object, and the second object is listed in the table. We use the Foundation object as the base because it provides a relatively stable base for the second object to be stacked upon, and lets us study the stacking performance for individual object types for the second object. 

% Our method outperforms or matches (within five trials) the PCA oriented bounding box baseline for 17/21 object types, demonstrating the advantage of our method. We analyze the cause of lesser performance for the remaining four object types. For the Rounded Bobble object, this object is nearly elliptical except for a small flat base. In the presence of noise, our learned algorithm, which relies on finding flat faces, is unable to detect the flat face. Detecting the maximal eigenvector should be easier to do under noise than classifying a set of contact points, so when the maximal eigenvector is orthogonal to the correct contact face, this heuristic should do better. For the remaining three objects (Cylinder Long, Foundation, and Rectangular Solid), these are long, narrow objects, whose contact face is again usually orthogonal to the principal axis. The learning based method suffers because it (say something about multimodality / incorrectness in plane prediction). Improving this aspect is an interesting direction for future work. 

% The maximal eigenvector heuristic used in PCA more frequently gives us the correct contact face in this case.

%   \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       %\includegraphics[scale=1.0]{figurefile}
%       \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%   \end{figure}
   

==> stacking_algorithm.tex <==
\begin{figure}[!t]
 \removelatexerror

\begin{algorithm}[H]
\caption{Stacking policy}
\label{alg: stacking_policy}
  \begin{algorithmic}[1]
\State \textbf{Input:} Segmented pointclouds $\{ X_i \}$, Object IDs $\{ i \}$, Centers of mass $\{p_i \}$, Object type labels $\{ A_i \}$, Max timesteps $T$, Visited object IDs array $V$, Rotation function $f$ \hspace{20mm}
\vspace{10pt}

\For{timestep $t$ in 1, ... , $T$}
    \State support\_block\_id = SampleSupportBlock($\{ A_i \}$, $\{ i \}$)
    \If{support\_block\_id is not None}:
        \State next\_block\_id = support\_block\_id
    \Else
        \State next\_block\_id = GetCapstoneBlock($\{ A_i \}$, $\{ i \}$)
    \EndIf
    \State centered\_pointcloud = $X_{\text{next\_block\_id}}$ - $p_{\text{next\_block\_id}}$
    \State $R$ = $f$(centered\_pointcloud)
    \State ApplyRotation(next\_block\_id, $R$)
    \State TranslateOntopExistingTower(next\_block\_id, $V$)
    \State StepEnvironmentAndUpdateVariables()
\EndFor
\end{algorithmic}
\end{algorithm}

\end{figure}
